"LazImpa": Lazy and Impatient neural agents learn to communicate efficiently

Previous work has shown that artificial neural agents naturally develop surprisingly non-efficient codes. This is illustrated by the fact that in a referential game involving a speaker and a listener neural networks optimizing accurate transmission over a discrete channel, the emergent messages fail to achieve an optimal length. Furthermore, frequent messages tend to be longer than infrequent ones, a pattern contrary to the Zipf Law of Abbreviation (ZLA) observed in all natural languages. Here, we show that near-optimal and ZLA-compatible messages can emerge, but only if both the speaker and the listener are modified. We hence introduce a new communication system, "LazImpa", where the speaker is made increasingly lazy, i.e. avoids long messages, and the listener impatient, i.e.,~seeks to guess the intended content as soon as possible.

==> PLAN.tex <==
\rahma{Suggested plan:}
\begin{itemize}
    \item \cite{chaabouni2019antiefficient} demonstrated how standard NN agent, when trained using standard training techniques to play a standard reconstruction game, develop an antiZLA-like distribution. This observation is robust to different hyper-parameters change. In this work, we will first reproduce prior work and add new insights about how emergent languages work then introduce our new setting (that is biologically plausible: this I need to look into a literature  that I am not familiar with) that forces the emergence of efficient (and stable?) languages.
    \item Experimental Framework:
    \begin{itemize}
        \item The Game: emergent language is usually studied using reconstruction games~\citep{chaabouni2019antiefficient,havrylov2017emergence}. We too, use such setting. Explain how, as you did, a reconstruction game works. 
        \item Optimization: in both cases we use the hybrid training (Backprob Listener and Reinforce Speaker).
    \end{itemize}
    \item ANTI-EFFICIENT PHENOMENA  IN EMERGENT COMMUNICATION:  reconstruction + further analysis
    \begin{itemize}
        \item Standard training: this would be the agent  architecture section that you described
        \item Results:
        \begin{itemize}
            \item We are able to reproduce the prior work (refer to the anti-ZLA figure).
            \item We also provide other analysis, namely the information content: discuss how non-informative these symbols are. Conclusion: actually agents are using efficient code with a lot of garbage (you can even refer in the appendix to how languages follow ZLA-like distrubution when you remove the non-informative symbols).
            \item Based on these results we introduce our new setting
        \end{itemize}
    \end{itemize}
    
        \item NEW  MODEL LEADING TO AN EFFICIENT COMMUNICATION: 
        \begin{itemize}
            \item Lazy Speaker and Imp. Listener
            \item Results: (1) position of the information (as expected) (2) ZLA (cool) (3) how close it is to Natural languages. Mention that on top of being efficient, it makes the training  more stable (refer to this in the appendix).
            \item Ablation study:
            \begin{itemize}
                \item Only Imp. Listener: Informative but long.
                \item Only Lazy Speaker: very hard to make it work.
            \end{itemize}
        \end{itemize}
\end{itemize}
\rahma{End of the suggestion}

==> old_main.tex <==


\newpage 


% OLD VERSON 
\newpage
\mathieu{OLD VERSION}

\section{Experimental framework}
\label{section:framework}       

We explore the properties of emergent communication in the context of referential games \cite{Lewis:1969} where agents have to cooperatively communicate in order to win the game. In the first part, we will describe the game setup and the optimization specificities.

\subsection{The game}

The game proceeds as follows:
\begin{itemize}
    \item Speaker network receives an input $i \in \mathcal{I}$ and generates a message $m$ of maximum length \verb+max_len+. The symbols of the message belong to a vocabulary $V=\{s_{1},s_{2},...,s_{\verb+voc_size+-1},\verb+EOS+\}$ of size \verb+voc_size+ where \verb+EOS+ is the `end of sentence' token indicating the end of Speaker's message. 
    \item Listener network receives and consumes the message $m$. Based on this message, it outputs $\hat{i}$.
    \item The two agents are successful if Listener manages to guess the right input, that is, if $\hat{i}=i$.
\end{itemize}

In our experiments, we make two main assumptions. First, the input space $\mathcal{I}$ is composed of 1000 one-hot vectors.  Inputs are not drawn uniformly from $\mathcal{I}$ but from a power-law distribution in order to match the distribution of words in natural languages. Consequently, the probability of sampling of the $k$-th most frequent input is: $\frac{1/k}{\sum_{j=1}^{1000}1/j}$ (see details in Appendix \ref{appendix:input_space}).
%\item \mathieu{OLD VERSION}
    %The couple of hyper-parameters (\verb+max_len+, \verb+voc_size+) are key in the study of the length statistics of the emergent communication. In order to limit the influence of these two parameters, we choose large values $\verb+max_len+=30$ and $\verb+voc_size+=40$ that are known to lead to anti-efficient communications.\rahma{How are they known? Mention the reference here. Say more it does not matter as any combination lead to anti-efficient code so we choose the closest setting to natural language.} \mathieu{ok}
Second, the couple of hyper-parameters (\verb+max_len+, \verb+voc_size+) are key in the study of the length statistics of emergent communications. \citet{chaabouni:etal:2019} showed that anti-efficient codes actually occur for any tested combination of those parameters. We thus chose $\verb+max_len+=30$ and $\verb+voc_size+=40$ which is the closest setting to natural languages we studied. To ensure the robustness of our systems, we will discuss at the end of the paper the influence of those assumptions (see Appendix \ref{appendix:assumption_analysis}).

In our analysis, we will only consider the successful runs, i.e. the runs with a uniform accuracy strictly higher than 97\% over all possible 1000 inputs. %The accuracy is weighted by the frequency of each of the 1000 inputs. In average, $\geq$97.5\% of the inputs are well communicated at the end of the training.

\subsection{Optimization}

The setting, which can be seen as a discrete auto-encoder, cannot be differentiated directly, as the latent space is discrete. Gumbel-softmax (\citet{Maddison:2016}, \citet{Jang:2016}), REINFORCE \cite{williams:1992} and an hybrid between REINFORCE for Speaker and classic back-propagation for Listener \cite{schulman:2015} are commonly used. We use the latter method as it has been considered as the most robust method by recent work \cite{chaabouni:etal:2019}.

\dpx{we need here a better explanation of what this mix is, and whether there are any hidden hyperparameters here, and if yes, how they are found. I suspect strongly that there is a hidden temperature coeficient here, that could become more explicit and be a part of the sloppy/lazy speaker, and even manipulated according to the schedule}

%\mathieu{BEFORE}
%We use the cross-entropy loss for the training. The parameters of Listener are merely optimized via back-propagation. Since the computation of the gradient w.r.t. to Speaker is impossible in practice, it is approximated by a Monte-Carlo integration calculated over samplings of the messages \mathieu{May I put an explanation of the optimization ? Appendix ?}\rahma{I think it is nice to have an equation summarizing the procedure. You can also have  the running mean and the entropy maximization in one equation.}. We use a running mean baseline to reduce the variance of this estimate \mathieu{CITE}. In addition, we promote exploration by adding a term in the loss that favors Speaker's high entropy. Eventually, the gradients are passed to the Adam optimizer with a learning rate that follows a simple decreasing scheduling.
%\bigbreak
We use the cross-entropy loss $\mathcal{L}$ for the training. The training task consists in minimizing the expectation of the cross-entropy loss $\mathbb{E}[\mathcal{L}(i,L(m))]$ where $L(m)$ is the output distribution of Listener that takes the message $m$ as input. The expectation is computed w.r.t the joint distribution of the inputs and the message sequences.  Let's denote $\theta_{L}$ and $\theta_{S}$ Listener and Speaker parameters. The optimization task requires to compute the gradient $\nabla_{\theta_{S}\cup\theta_{L}}\mathbb{E}[\mathcal{L}(i,L(m))]$ w.r.t both to the parameters of Speaker and Listener. An unbiased estimate of this gradient is:

\begin{equation}
\begin{split}
      \mathbb{E}[&\underbrace{\nabla_{\theta_{L}}\mathcal{L}(i,L(m;\theta_{L}))}_{(A)} + \\ &\underbrace{\{\nabla_{\theta_{S}}(\mathcal{L}(i,L(m;\theta_{L})\} - b)\log P_{S}(m|\theta_{S})}_{(B)}]
\end{split}
\end{equation}

where $\{.\}$ is the stop-gradient operation, $P_{S}(m|\theta_{S})$ the probability that Speaker generates the message $m$ and $b$ the running-mean baseline used  to reduce variance \cite{williams:1992}.
\bigbreak
The gradient (A) w.r.t $\theta_{L}$ is found via back-propagration. Since the computation of the gradient (B) w.r.t $\theta_{S}$ is impossible in practice, it is approximated by a Monte-Carlo integration calculated over samplings of the messages. In addition, we promote exploration by adding a penalty term in the loss $\mathcal{L}(.)$ that favors Speaker's high entropy. Eventually, the gradients are passed to the Adam optimizer \cite{kingma2014adam}. 

\dpx{aha!! this is where the hidden exploration hyper parameter is; this should be integrated in equation (1) and be attributed to the exploration/exploitation tradeoff of the speaker. Also, it would be very interesting to see whether a scheduling of this one could make the agents even more efficient -- avoiding the emergence too early of 'favorite' symbols. }

\bigbreak
We use the EGG toolkit \citep{Kharitonov:etal:2019}. For reproductibility, the code link will be available upon acceptance and the set of hyper-parameters used is presented in Appendix \ref{appendix:experimental_settings}.

\subsection{Reference distributions}

We compare the emergent languages to the reference distributions introduced in \citet{chaabouni:etal:2019}. We provide below a brief description of the different references, however, we invite readers to refer to \citet{chaabouni:etal:2019} for more details.

\paragraph{Optimal Code} \citep{Cover:Thomas:2006}: guarantees the shortest average message length for a given  \verb+max_len+ and \verb+voc_size+. To do so, we deterministically associate the shortest  messages to the most frequent inputs. See \citet{FerrerICancho:etal:2013} for more details about the derivation of Optimal Code.

\paragraph{Monkey Typing} \citep{miller:1957}:
Consists of creating messages by uniformly drawing symbols till sampling \verb+EOS+. Despite its randomness, this reference follows a ZLA-like distribution, %Following \citet{chaabouni:etal:2019}, we consider this reference as a less strict benchmark for network efficiency.
which originates from the fact that the probability of sampling short messages is larger than the one of longer messages. We hence consider Monkey Typing as a less strict benchmark for network efficiency. %Refer to \citet{chaabouni:etal:2019} for further details about its derivation

\paragraph{Natural Language}: We also compare  emergent languages with several human languages. In particular, we consider the same languages introduced in \citet{chaabouni:etal:2019} (i.e. English, Arabic, Russian and Spanish). These references consist of the mapping  from the frequency of the top $1000$ most frequent words  in each language to their length (approximated by the number of characters of each word).


\section{Anti-efficient phenomena in emergent communication}
\label{Section:anti-eff}

The first part of our work consists in reproducing and characterizing the anti-efficient phenomena that occur in emergent communication. Our goal is to spot recurrent tendencies in the emergent communication that can further lead to an adaptation of standard models. 

\subsection{Agent architecture}

For this first part, the two agents are standard single-layer LSTMs. First, Speaker's inputs are mapped by a linear layer into an initial hidden state of Speaker's LSTM cell. Then, the message $m$ is generated symbol by symbol: the current sequence is fed to the LSTM cell that outputs a new hidden state. Next, this hidden state is mapped by a linear layer followed by a softmax to a Categorical distribution over the vocabulary. During the training phase, the next symbol is sampled from this distribution. During the testing phase, the next symbol is deterministically selected by taking the argmax of the distribution.


Secondly, Listener receives the entire message $m$. Until the \verb+EOS+ token is seen, Listener consumes the symbols one by one. In the end, the final hidden state is mapped to a Categorical distribution over the input indices (linear layer + softmax). This distribution is then used during the training to compute the cross-entropy loss w.r.t. the ground truth $i$. During the testing phase, we take the argmax of the distribution as candidate.

\subsection{Results}

\citet{chaabouni:etal:2019} highlighted how standard agents develop anti-ZLA languages. 
That is, the longest messages are associated to the most frequent input. We start with reproducing these results then  provide a better intuition of the functioning of this phenomenon.

\paragraph{Anti-ZLA communications.}

%\bigbreak
As shown in Figure~\ref{fig:ZLA} (green curve),  
%As detailed in Appendix \ref{appendix:anti_ZLA}, 
we reproduce \citet{chaabouni:etal:2019}'s result and  obtain anti-efficient emergent languages. In particular, our emergent languages have length distributions almost constant and equal to the maximum length we set (\verb+max_len+). They are even less efficient than the Monkey Typing distribution (a random baseline) (see details in Appendix \ref{appendix:anti_ZLA}). %Therefore, the distributions of lengths in emergent languages are very different from those of natural languages: it does not follow ZLA and more generally tend to use messages as long as possible. 
To bring some insights about this length anti-efficiency, we analyzed how the average length of the messages evolves during the training. In Appendix \ref{appendix:learning_path}, we demonstrate that the agents tend to explore long messages very quickly. At the beginning of the learning process, the messages are short and the accuracy is low. Then, when and only when the messages become long, communication starts to become successful. These results suggest that using long messages is key for the agents to converge even though shorter messages are sufficient to succeed in the game. 

\dpx{The paper is a bit difficult to read; the results of section 3 are in figures at the end of the paper; analysis methods are introduced in the middle. This reflects the history of the internship, but in a paper, you are allowed to reorder the materials to make it easier to follow. I think it would be more efficient to merge these section 3 and 4. In an "architecture" section, you could present the two architectures, the standard vs the impatient listeners. In a "loss" or "training" section, the standard vs the impatient loss plus the adaptive one. This would make it easier to reintegrate the entropy loss in the formula and present it as a regularization for the speaker. You could also introduce in an "analysis" section your new way of measuring positional encoding (it is, right now, in the awkwardly named section "Anti-efficient allocation of the information" in the middle of results). This is a method and should appear as such. Then a "result" section presents both the old results and the new jointly , as they are in the figure 3. Also, Figure 6 should appear before, no?}

\paragraph{Anti-efficient allocation of the information. }

We also study how informative the messages symbols are. Concretely, we consider a symbol to be informative if
%Paradoxically, even if the messages are long, only a small part of the messages are informative, that is, has an influence on Listener's predictions. To measure if a symbol is informative, we applied the following protocol: we consider that a symbol is informative if 
changing it randomly has an effect on Listener's prediction. In other words, if it is crucial for the communication. Formally, let's take the message $m=(m_{0},...,m_{t})$ associated to the ground truth input $i$. To evaluate the information contained in the symbol $m_{k}$, we substitute it randomly by drawing another symbol $r_{k}$ uniformly from the vocabulary (except the \verb+EOS+ token). Then, we feed this new message $\Tilde{m}=(m_{1},...,r_{k},...,m_{t})$ into the Listener that outputs $\Tilde{o}_{m,k}$ (index $m$ means that the original message was $m$, index $k$ means that the $k^{th}$ symbol of the original message has been changed). We define $\Lambda_{k,m}$ a boolean score that evaluates whether the symbol changed at position $k$ has an impact on the prediction, such that  $\Lambda_{k,m}=\mathbf{1}(\Tilde{o}_{k} \neq i)$. If $\Lambda_{k,m}=1$, the $k^{th}$ symbol of message $m$ is considered as informative. If $\Lambda_{k,m}=0$, it is considered as non-informative.


%If this substitution has no effect on the prediction, we consider that the symbol is non-informative. On the contrary, if Listener fails to predict the right output after this substitution, we consider that the symbol is informative. 
This test allows us to both estimate the proportion of symbols that are informative in a communication and localize the informative and non-informative parts of the message. Indeed, we assign a score $\Lambda_{k,.}$ on each position that counts the proportion of informative symbols over all the messages at position $k$:

\begin{equation}
    \Lambda_{k,.}=\frac{1}{N}\sum_{m}\Lambda_{k,m}
\end{equation}
where $N=1000$ is the total number of messages.

In Figure \ref{fig:position_compa}, we plot spectra that show how `informative' the different positions are by introducing a gray gradient that maps $\Lambda_{k,.}$ to a color that goes from black ($\Lambda_{k,.}=0$) to white ($\Lambda_{k,.}=1$).

%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{0.8\textwidth}
%    \includegraphics[scale=0.3]{figures/spectrum_N_HQ.png}
%    \hfill
%    \includegraphics[scale=0.27]{figures/gradient_HQ.png}
%    \end{subfigure}
    
%    \caption{Proportion of informative symbols averaged across all emergent messages. Each box represents the proportion of informative symbols at a given position mapped to a color according to a black to white gradient. The vertical red line marks the average length of the messages across the different runs. \rahma{remove it and refer to Fig8 (a)}}
%    \label{fig:pos_N}
%\end{figure}

Looking  at the spectrum of standard agents in Figure \ref{fig:posN}, we can make two striking observations. First,  only a very small part of the messages are actually informative (in average 18\%). Therefore, even if  long messages seem necessary for the agents to converge, most of the symbols are actually useless. Second, in all our experiments, the information is localized at the very end of the messages. %Consequently, all the messages are composed of a long part at the beginning that is useless and a short part that is informative. 
Actually, in Appendix \ref{appendix:info_analysis}, Figure \ref{fig:info_ZLA}, we observe that, if we restrict the messages to their informative parts (i.e. removing symbols of $\Lambda_{k,.}=0$), the length statistics follow a ZLA-like distribution similar to natural languages.
%We report in Appendix \ref{appendix:info_analysis}, Figure \ref{fig:info_ZLA}, the average length of informative parts as a function of the input frequency rank and compare it to the word's length distributions of natural languages. We observe that the length order of magnitude is the same for the emergent communications and the natural languages. Moreover, we see that the length distribution of the informative parts begins to follow ZLA. See Appendix~\ref{appendix:info_analysis} for more details. 
%\bigbreak
In other words, agents are actually using efficient code but also add a lot of ``garbage'' symbols. We aim to adapt our communication system to lead the agents to keep only the informative parts of their code.



%\begin{figure}
%  \begin{subfigure}{.44\textwidth}
%  \centering
%  % a) normal
%  
%  \includegraphics[scale=0.5]{figures/p%ositional_spectrum_N.png}  
%  \caption{Classic listener}
%  \label{fig:pos_spectrum_classic}
%  \end{subfigure}
%  \begin{subfigure}{.44\textwidth}
%  \centering
%  % b) impatient
%  \includegraphics[scale=0.5]{figures/positional_spectrum_imp.png}  
%  \caption{Imp. Listener}
%  \label{fig:pos_spectrum_imp}
%  \end{subfigure}
%  \begin{subfigure}{.1\textwidth}
%  \centering
%  % b) impatient
%  \includegraphics[scale=0.5]{figures/positional_gradient.png}  
%  \end{subfigure}
  
%    \caption{Positional spectra of the information in the emergent languages. Each position is assigned a value equal to proportion of informative symbols at this position over all the messages of 3 different random seeds \rahma{Why not all the 6 seeds used in the remaining analysis?}. Each value is mapped to a color according to a gradient that goes from 0 (black) to 1 (white). (a) is the position spectrum of the classic listener ; (b) the positional spectrum of the Imp. Listener.\rahma{add the same figure  for the impatient + regularization: c'est le modele qui nous interesse le plus.}}
%    \label{fig:spectrum}
%\end{figure}

\section{New communication system leading to an efficient communication}
\label{Section:Impala}

Based on these observations, we introduce small variations on agents in order to get an efficient communication. In this section, we present both the new communication system and the results we obtained. We will show that our new system lead to ZLA code as efficient as natural language. 
Finally, we will analyze the effect of the made modeling choices.

\subsection{Updates of the agents model}
\label{subsection:Impala_model}

In order to get an efficient communication, we consider a two-step strategy:

\begin{enumerate}
    \item Modify agents in order to force the system to place the informative symbols at the beginning of the messages.
    %\item Apply an adaptive regularization that allows to find a right trade-off between length exploration and concision.
    %\rahma{clarify that: between  length regularization and informativeness?}
    \item Apply an adaptive regularization that first lets the system explore long messages and then find the right trade-off between concision and informativeness.
\end{enumerate}

\subsubsection{``Imp. Listener''}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.35]{figures/LSTM_modele_HQ.png}
    \caption{``Imp. Listener'' architecture. The agent is composed of one LSTM cell and one linear layer followed by a softmax. ``Imp. Listener'' generates a prediction at each time step.%The LSTM cell generates a hidden state for all the symbols of the message $m$ which are then mapped to a Categorial distribution over the input indexes by the linear layer and the softmax.
    }
    \label{fig:impatient_listener_model}
\end{figure}

First, we introduce a new model for Listener, which we further call ``Imp. Listener'' (for Impatient Listener). The idea behind the ``Imp. Listener'' is to create a Listener model that tries to guess the right output as soon as possible. In the standard architecture, Listener reads the message $m$ entirely before outputting a candidate. With the ``Imp. Listener'' we update this model by taking advantage of the recurrent property of the LSTM. As shown in Figure \ref{fig:impatient_listener_model}, the ``Imp. Listener'' works as follows: the agent receives the entire message $m=(m_{0},...,m_{t})$ composed of $t+1$ symbols. Then, the LSTM cell consumes each symbol from position $0$ to $t$ generating $t+1$ hidden states $(h_{0},...,h_{t})$ for all the different positions of the message. All these hidden states are then mapped to a Categorical distribution over the input indices using a shared single linear layer followed by a softmax. Eventually, we get a sequence of $t+1$ distributions $L(m)=(L(m)_{0},...,L(m)_{t})$, one for each position of the message. Note that a similar process can be adapted for any recurrent and causal network Listeners.


To force Listener to guess the correct candidate right from the beginning, we introduce an updated loss $\mathcal{L}_{imp}$ that includes all the intermediate distributions. For an input $i$ and a sequence of intermediate distributions $L(m)=(L(m)_{0},...,L(m)_{t})$, the loss becomes:

\begin{align}
    \mathcal{L}_{imp}(i,L(m))=\frac{1}{t+1}\sum_{k=0}^{t}\mathcal{L}(i,L(m)_{k})
\end{align}

The earlier Listener predicts the correct output, the larger the reward is. Consequently, we expect the information to be introduced right from the beginning of the messages.


At test time, we only take the argmax of the distribution generated by Listener when it reads the \verb+EOS+ token.

\subsubsection{Adaptive regularization}

The first step is supposed to force the agents to introduce informative symbols at the beginning of the messages. Nevertheless, to this point, nothing has been done to shorten the messages. Because length regularization lead to an unstable training in  \citep{chaabouni:etal:2019}, we consider here an adaptive one. The idea is to first let the system explore long and discriminating messages and then, once it reaches good enough communication performances, we apply a length pressure. Therefore, we model a feedback between the two agents by introducing a regularization parameter $\alpha$ that depends on the commmunication accuracy. With $|m|$ the length of the message associated with the input $i$, $\mathcal{L}$ the loss of the system and 
`$\text{acc}$' the estimation of the accuracy (proportion of inputs correctly communicated weighted by appearance frequency), the new loss becomes:

\begin{align}
    \mathcal{L}_{reg}(i,L(m))=\mathcal{L}(i,L(m)) + \alpha(\text{acc})|m|
\end{align}


To schedule this two-step training, we model $\alpha$ as shown in Figure \ref{fig:alpha_model}.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{figures/alpha_sched_HQ.png}
    \caption{Scheduling of the regularization parameter $\alpha$ as a function of the accuracy. See the mathematical description of the curve shape in Appendix \ref{appendix:reg}}
    \label{fig:alpha_model}
\end{figure}

The regularization is mainly composed of two branches. Firstly, the regularization is almost null: we let the system use long messages in order to reach high accuracies (\textbf{convergence step}). Secondly, when the two agents become successful, we start to force the system to shorten the messages (\textbf{ablation step}). If the information is well set at the beginning of the messages with the introduction of the ``Imp. Listener''  we expect the system to easily shorten the messages. As this regularization is applied on Speaker side, we refer to this variation as ``Reg. Speaker'' (for Regularized Speaker).

\subsection{Results}
\label{subsection:Impala_results}

We train our Speaker/Listener agents to solve the reconstruction game after introducing both modifications. We refer to this final model as (Reg. Speaker + Imp. Listener). In this section, we compare the results of this new system with the standard one. All the instances of (Reg. Speaker + Imp. Listener) have been successful (i.e, more than 97\% of all inputs are correctly reconstructed independently of  their frequency). % , that is, the accuracy within a batch was higher than 99\% (the accuracy is weighted by the frequency of the input, in average, this score means that more than 97.5\% are well communicated). 

% OLD Moreover, on top of being successful, our new model provides a more stable training even in the presence of length regularization (see details in Appendix \ref{appendix:convergence}).

\mathieu{NEW}
\paragraph{Stability.}
On top of being successful, our new system provides a more stable training even in the presence of length regularization. We compare the convergence results of: (Standard Speaker + Standard Listener), (Imp. Listener + Standard Speaker), (Imp. Listener + Regularized Speaker) for several initializations (see curves in Appendix \ref{appendix:convergence} Figure \ref{fig:convergence}). The convergence dynamic is sensitive to the initialization but in the end, the three systems converge every time.

\begin{table*}[h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{|c||c|c|c|}
    \hline
& Std. Listener & Imp. Listener + Std. Speaker & Imp. Listener + Reg. Speaker \\ \hline
\rho_{stab} & 1.22\times10^{-3} \pm9.9 \times 10^{-4} & 1.49\times10^{-4}  \pm 7.5\times10^{-5} & 1.00\times10^{-4} \pm 5.1\times10^{-5} \\ \hline
\end{tabular}
\end{adjustbox}
    \caption{Average MSE between the original and smoothed training curve quantifying the local variations of the training curve}
    \label{tab:stability_m}
\end{table*}

%\bigbreak
However, we observe a gain of stability when introducing Imp. Listener. Indeed, a lot of accuracy drops occur when training standard agents compared to both (Imp. Listener + Standard Speaker) and (Imp. Listener + Regularized Speaker). We quantify the stability by introducing a coefficient $\rho_{stab}$ that measures the local variations of the accuracy curves. This coefficient computes the mean square error between the original accuracy curve and the smoothed curve obtained by averaging 10 consecutive accuracy values: 

\begin{equation}
    \rho_{stab} = \frac{1}{n}\sum_{i=1}^{n}(f(i)-\Tilde{f}(i))^{2}
\end{equation}
where $n$ is the total number of episodes, $f(.)$ the accuracy curve, $\Tilde{f}(.)$ the curve obtained by averaging $f(.)$ over with 10 consecutive values. The lower $\rho_{stab}$ the smoother the training curve is.

Results are reported in Table \ref{tab:stability_m}. $\rho_{stab}$ for systems with Imp. Listener are significantly smaller than the one with Standard Listener confirming that introducing Imp. Listener leads to more stable trainings. It is important noticing that, contrary to \citet{chaabouni:etal:2019}'s setting, the addition of the adaptive regularization on the Speaker has no negative effect on the convergence success and stability. 


\paragraph{ZLA communication.}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.5]{figures/fig3_ZLA_HQ.png}
    \caption{Average message length across successful runs as a function of input frequency rank. The blue curve refers to the system \{Reg. Speaker + Imp. Listener\}, the green curve the system with standard agents (light intervals show 1 standard deviation). The grey curve refers to the Monkey Typing distribution and the purplr curve to Optimal Coding.} 
    \label{fig:ZLA}
\end{figure} 

\begin{figure*}[h]
    \begin{subfigure}[t]{.46\textwidth}
    \includegraphics[scale=0.47]{figures/compa_NL_HQ.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.46\textwidth}
    \includegraphics[scale=0.43]{figures/unigrams_HQ.png}
    \end{subfigure}
    \begin{subfigure}{1.\textwidth}
    \centering
    \includegraphics[scale=0.6]{figures/legende_nat_lang.png}
    \end{subfigure}
    \\
    \begin{subfigure}{.46\textwidth}
    \caption{Average message length across successful runs as a function of input frequency rank. For the sake of readability, the curves have been smoothed using a sliding average of 20 consecutive lengths, see the real curves in Appendix \ref{appendix:stat_NL}. The light blue interval shows 1 standard deviation for the emergent language distribution.}
    \label{fig:compa_len}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.46\textwidth}
    \caption{Average unigrams distribution across the messages ranked by unigram frequency. The light blue interval shows 1 standard deviation for the emergent language unigrams distribution.}
    \label{fig:compa_uni}
    \end{subfigure}
    \caption{Comparison of the Emergent Language statistics with natural languages.}
    \label{fig:compa_NL}
\end{figure*}

(Reg. Speaker + Imp. Listener) develops an efficient communication as presented in Figure \ref{fig:ZLA}. Indeed, the average length of the messages is significantly lower than the system with standard agents and Monkey Typing baseline. In addition, we see that the length distribution follows ZLA: the shortest messages are associated to the most frequent inputs (see Appendix \ref{tab:quant} for a quantitative support of this observation). 

%In Figure  \ref{fig:ZLA}, we also report the length distribution that would be obtained by randomly typing the symbols (Monkey Typing). %Each time the writer types a symbol, it has a $\frac{1}{voc\_size}$ probability of writing the \verb+EOS+ token. The end of a message appends when the \verb+EOS+ is output by the writer.
%We see that the communication that emerges from our model is significantly more efficient that the one of a random Speaker.

However, we can notice that, even if the communication is very efficient, we do not get the optimal coding. The optimal coding is the set of messages that minimizes the length pressure while successfully discriminating the inputs given the vocabulary size. Theoretically, the agents should be able to reach this optimum. However, we observe on Figure \ref{fig:ZLA} that we get a sub-optimal solution.

\paragraph{Efficient allocation of the information.}
We also look at information allocation when experimenting with (Reg. Speaker + Imp. Listener) model. In Figure \ref{fig:posIRL}, we observe that this new model leads to a more efficient allocation of the information. In fact, Listener relies on 48.5\% of information compared to 18\% when using standard model. However, this also means that Listener still relies on less symbols than provided by Speaker (even if the latter is subject to a length cost). 
%In particular, Listener uses in average 2.67 symbols by message when the mean length of messages is 5.5. 
Interestingly, in contrast of standard agents, these useful symbols are localized in the first positions making the communication closer to animal communication. Both observations are also observed in human communication with uniqueness point (where listener human predicts speaker's intention before the end of the latter's message) \cite{marslen:1987} and animal communication \cite{mclachlan2020speedy}. Note that the presence of uninformative symbols provides a partial answer to the non-optimality of emergent languages observed in the previous part. Indeed, Listener uses in average 2.74 symbols which is quite close to the optimal coding (of average length 1.96), suggesting that the gap to optimality is mainly caused by Speaker. We investigate plausible sources of Speaker sub-optimality in Appendix \ref{appendix:min_length} and show that one  source is the non-uniform use of the unigrams (see Figure \ref{fig:compa_uni}). Nevertheless, Speaker still adds a few ``garbage`` symbols for a convergence purpose. We leave the analysis of reaching an optimal communication to future works.
 %Thus, we observe that the Imp. Listener works as expected: by trying to find the right candidate as soon as possible, it actually relies only on the beginning of the training.

%\begin{figure}[h]
%    \centering
%    \begin{subfigure}{0.8\textwidth}
%    \includegraphics[scale=0.3]{figures/spectrum_ILR_HQ.png}
%    \hfill
%    \includegraphics[scale=0.27]{figures/gradient_HQ.png}
%    \end{subfigure}
%    \caption{Proportion of informative symbols averaged across all emergent messages. Each box represents the proportion of informative symbols at a given position mapped to a color according to a black to white gradient (black=0 ; white=1). The orange line marks the average length of the messages. \rahma{I still think you can come up with a better representation.}  \rahma{also to remove and just refer to figure8(c)}} 
%    \label{fig:position_IRL}
%\end{figure}




\subsection{Comparison with natural languages}
\label{subsection:compa_natL}

%With this model, we actually obtain a communication that is statistically close to natural languages. In Figure \ref{fig:compa_NL}, 
We compare two statistical properties of the emergent language and natural languages, namely, length and unigram distributions. Results are shown in Figure \ref{fig:compa_NL}. In addition of the ZLA property, we see in Figure \ref{fig:compa_len} that the lengths of the messages in the emergent communication are, in average, analogous to the words lengths in natural languages (see Appendix \ref{tab:quant} for a quantitative support of this observation). Regarding unigram distribution of emergent languages, in Figure \ref{fig:compa_uni}, we can notice that it is as skewed. This is an unexpected property (we would rather expect a uniform distribution) that actually fits well the distributions of unigrams observed in natural languages. 

\subsection{Effect of the modeling choices made}
\dpx{should not this be called "ablation studies"?}
\label{subsection:model_choices}

\begin{figure*}[h]
    \begin{subfigure}[t]{.48\textwidth}
    \includegraphics[scale=0.44]{figures/learning_path.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.48\textwidth}
    \includegraphics[scale=0.5]{figures/fig5B_ZLA_compa_model_HQ.png}
    \end{subfigure}
    \begin{subfigure}{1.\textwidth}
    \centering
    \includegraphics[width=1.\textwidth]{figures/legende_modele_compa.png}
    \end{subfigure}
    \\
    \begin{subfigure}{.46\textwidth}
    \caption{Joint evolution of the accuracy and mean length for the different models. Each point shows the couple (mean$\_$lenght,accuracy) of one training episode. Arrows represent the average joint evolution of the two variables.}
    \label{fig:compa_learning_path}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.46\textwidth}
    \caption{Average message length as a function of input frequency rank for the different systems. Light color intervals show 1 standard deviation.}
    \label{fig:compa_length}
    \end{subfigure}
    \caption{Models comparison. In both the two figures, the green curve refers to the system (Standard Speaker + Standard Listener), the red curve to the system (Reg. Speaker + Standard Listener), the orange curve to the system (Standard Speaker + Imp. Listener), the blue curve to the system (Reg. Speaker + Standard Impatient)} 
\end{figure*}

We have just seen that our new communication model allows agents to develop an efficient and ZLA-obeying language whose statistical properties are close to those of natural languages. In this section, we analyze the effects of the modeling choices we have made.

%\mathieu{OLD}
%We first look  the effect of length regularization. 
%Figure \ref{fig:compa_learning_path} shows the joint evolution of the mean length of the messages and the  accuracy. For the system \{Regularized Speaker + Imp. Listener\}, we see that there are two steps during the training. First, the system explores long messages while being more successful. Secondly, when a high accuracy is reached ($\sim 0.98$) the regularization starts becoming effective and the mean length is decreasing: the communication becomes very efficient. Naturally, we can wonder if the efficiency is only due to the introduction of the adaptive regularization. However, we see in Figure \ref{fig:compa_length} that the ablation step is impossible with a standard listener: the system \{Regularized Speaker + Standard Listener\} still uses long messages. More generally, as shown in \cite{chaabouni2019antiefficient}, it is hard to regularize systems with a standard listener. We can suggest that the fact that Listener relies on the end of the messages makes the regularization hard to work.  Consequently, the ability for the Listener to guess the right candidate as soon as possible is also key to obtain an accurate and efficient communication. 


%As shown in Table.\ref{table:position_table}, the introduction of the Imp. Listener has a tremendous effect on the allocation of the information. While less than 20\% of the symbols are informative for the systems with a Standard Listener, we see that almost all the symbols become informative with the introduction of the Imp. Listener.

%We see on Figure \ref{fig:compa_length} that the communication emerging from the system \{Standard Speaker + Imp. Listener\}, starts to follow the ZLA, but the number of symbols used remains anti-efficient. In the end, it is the combination of the Regularized Speaker and the Imp. Listener that leads to an efficient communication that follows ZLA. 

We first look the effect of length regularization. Figure \ref{fig:compa_learning_path} shows the joint evolution of the mean length of the messages and the accuracy. For the system (Reg. Speaker + Imp. Listener), we see that there are two steps during the training. First, similarly to the standard system, (Reg. Speaker + Imp. Listener) explores long messages while being more successful (convergence step). Secondly, when a high accuracy is reached ($\sim 0.98$) the regularization starts becoming effective and the mean length decreases: the communication becomes efficient (ablation step). As shown in Figure \ref{fig:compa_length}, the introduction of the regularization for the system (Reg. Speaker + Imp. Listener) has a strong effect on the length statistics compared to the system (standard Speaker + Imp. Listener) where we only note the convergence step. Naturally, we can wonder if the efficiency is only due to the introduction of the adaptive regularization. However, we see in Figure \ref{fig:compa_learning_path} that the system (Reg. Speaker + standard Listener) follows the same learning path as the standard system. In particular, once an high accuracy is reached, the ablation step is impossible. Consequently, we see in Figure \ref{fig:compa_length} that the length statistics of the two models is equivalent and that the regularization is not efficient. More generally, it is hard to introduce a length regularization when experimenting with standard Listener \citep{chaabouni:etal:2019}. 

\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{.3\textwidth}
    \includegraphics[width=1.\textwidth]{figures/spectrum_N_HQ.png}
    \caption{Standard agents}
    \label{fig:posN}
    \end{subfigure}
    \begin{subfigure}[t]{.3\textwidth}
    \includegraphics[width=1.\textwidth]{figures/spectrum_IL_HQ.png}
    \caption{Std. Speaker + Imp. Listener}
    \label{fig:posIL}
    \end{subfigure}
    \begin{subfigure}[t]{.3\textwidth}
    \includegraphics[width=1.\textwidth]{figures/spectrum_ILR_HQ.png}
    \caption{Reg. Speaker + Imp. Listener}
    \label{fig:posIRL}
    \end{subfigure}
    \begin{subfigure}[t]{.06\textwidth}
    \includegraphics[width=0.5\textwidth]{figures/gradient_HQ.png}
    \end{subfigure}
    
    \caption{Proportion of informative symbols of the different systems averaged across all emergent messages of successful runs. Each box represents the proportion of informative symbols at a given position mapped to a color according to a gray gradient (black=0 ; white=1). The red lines mark the average length of the messages}
    \label{fig:position_compa}
\end{figure*}

How can we explain the difference in behavior between Standard and Imp. Listener ? We can suggest that this is due to the allocation of information in the messages. As shown in Figure \ref{fig:position_compa}, we see that contrary to Standard Listener (\ref{fig:posN}) that only relies on symbols at the end of the messages (in average 5.4), the introduction of Imp. Listener (\ref{fig:posIL} and \ref{fig:posIRL}) crucially changes the symbols to which Listener relies on. These symbols are fewer (in average 2.6) and localized at the beginning of the messages. This move enables the introduction of the regularization for the Speaker that removes the unused parts of the messages at the end of the training. By comparing Figure \ref{fig:posIL} and \ref{fig:posIRL}, we see that the introduction of the regularization has no effect on the position of the information. Meanwhile, we see that the average length of the messages significantly decreases with the regularization (in average from 19.3 to 5.49) leading to an efficient communication. 

In the end, it is a combination of Imp. Listener and the adaptive regularization that allows to get an efficient communication.

%\section{Compositionality (titre à déterminer)}

%With this agents model, we manage to get a very efficient communication that follow some natural language properties: ZLA-like distribution of the message lengths, skewed distribution of the vocabulary. Then, we want to see if this gain of efficiency (compared to the previous models) leads to a gain of structure in the communication i.e. the emergence of a grammar. Consequently, we study a derived experiment in order to test the computationally of the emergent language.

%\subsection{Update of the experiment}

\section{Conclusion}
\rahma{still darfty but this is the idea}\\
We demonstrated that standard communication models, where standard Speaker and Listener LSTMs are trained to solve a simple reconstruction game, lead to long messages, close to the maximal threshold. Surprisingly, if these messages are long, LSTM agents rely only on a small number of informative messages’ symbols, located at the end. Based on these observations, we introduce a new communication system, (Reg. Speaker, Imp. Listener). On one hand, Reg. Speaker is obtained by introducing a cost on messages length once the communication is successful. On the other hand, Imp. Listener, contrary to the standard one, aims to succeed in the game as soon as possible, by predicting Speaker's input at each message position.

We show that both modifications are \emph{necessary} for the emergence of ZLA-like protocol, as efficient as natural language. For example, Reg. Speaker alone will fail to shorten the messages, which highlight the importance of the ``impatience/predictive'' mechanism. The importance of the latter in language acquisition is still subject to debate, but many prior works had pointed to its necessity to human language understanding \citep[e.g.][]{clark:2013,friston:2010}. Our results confirm that \rahma{TODO}. Also, interesting, if this mechanism makes the emergent language more efficient, the latter would be still far from natural language. In other words, efficiency needs constraints \emph{both} on Speaker and Listener sides. In that sense, our results are in line with many previous works that state that our language is shaped by the pressures toward (1) maximizing informativeness (ensured by the predictive/impatience mechanism) and (2) minimizing complexity (encoded by the length regularization) \citep[see][for a survey]{Gibson:etal:2019}. (\rahma{todo: discuss that our system is easy to use: general and stable, somewhere}).\dpx{introduce perhaps the idea that the scheduling of the speaker mimics the babbling phase of the infant who explore its phonetic space before restricting its messages to those of the native language?}

Finally, our work highlights the importance of introducing the right constraints in the communication system. Indeed, to construct automated agents that would eventually interact with humans, we need to introduce constraints, that if task-agnostic, allow the emergence of more ``human-like'' communication. 

\dpx{This work opens several lines of research. One would be to push the regularization losses even further to insure robust efficiency in all situations. Indeed, while our results show human-level efficiency, our agents do not reach optimal coding. A training regime ensuring optimal coding would have a variety of applicaitons.}

A second line of research would be to apply this system to other games or NLP problems and study how it affects other properties of the emergent language such as regularity or compositionality.


%\rahma{WIP}\\
%1. demonstrated that standard communication models, where Speaker and Listener neural networks are trained to solve a simple reconstruction task, lead to long messages, close to the maximal threshold. \\

%2. show that if neural networks use long messages, they only use a small number of messages' symbols. This information is located at the end of this  message. \\

%3. Based on these observation we introduce a new communication system Reg. Speaker and Impatient Listener. It consists of modifying the standard emergent-communication system by (1) and (2). Both constraints are biologically plausible.\\

%4. We show that the emergent language is ZLA and close to natural language. Also, it is stable and general\\

%5. Both constraints are important, without (1)  ... and without (2) ....\\



%We demonstrated that standard communication models, where Speaker and Listener neural networks are trained to solve a simple reconstruction task, lead to long messages, close to the maximal threshold. Interestingly, follow-up experiments show that if neural networks use long messages, they only use a small number of messages' symbols. This information is located at the end of this  message. We connect this non-informative long messages to the absence of predictive mechanism in the listener. A mechanism that is argued, even if still subject to a debate, to be necessary to understand language \citep{clark:2013,friston:2010}. We hence introduce an Impatient listener that .... Interestingly, we show that this constraint alone, if is makes the information at the beginning the message enabling Impatient listener to predict Speakers inputs before the end of the messages. However,  the messages are still long. We hence, add .... introducing Regularized Speaker. this constraint applied  in the presence of  Imaptient Listener, enables easy-to-optimize system, contrary to what is found when applied on standard listeners. Our new communication  system (Reg. Speaker + Impatient Listener) enables the emergence of an efficient communication protocol very close to natural languages.  Both constraints are important: Indeed (1) alone ... and (2) alone .... This result is inline with prior work that suggest that languages are shaped by a balance between (1) and (2) (cite chaabouni, semantic ... , ramon? ... ) \\

%6. To be able to construct agents that would eventually communicate with humans, we should re-think on the needed constraints. Both our constraints are easy to introduce and leads to the development of more human-like communication.\\

%7. In future work, we want to apply this system on other games and study how it affects other properties of the emergent language such as regularity or compositionality.


==> old_results.tex <==
\section{Results}
\label{section:results}

\begin{table*}[h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{|c|c||c|c|c||c|c|}
    \hline
         Class & Code & $L_{uni}$ &$L_{weight}$& $p_{\alpha}$ & $L_{eff}$ & $\rho_{inf}$ \\
        \hline
         Emergent & Standard Agents & $29.6 \pm 0.4$ & $29.91 \pm 0.07$ & $>1-10^{-5}$ & $3.33 \pm 0.46$ & $0.11 \pm 0.02$  \\  
          & LazImpa & $5.49 \pm 0.67$ & $3.78 \pm 0.34$ & $<10^{-5}$* &  $2.67 \pm 0.07$ & $0.60 \pm 0.07$ \\  
         \hline
         \hline
         & Monkey Typing & $20.79 \pm 0.07$ & $20.76 \pm 0.08$ & 0.866 & / & / \\  
         References & Mean natural languages & $5.46 \pm 0.61$ & $3.55 \pm 0.14$ & $<10^{-5}$* & / & / \\
         & Optimal Coding & $2.96$ & $2.29$ & $<10^{-5}$* & $1.96$ & $1.00$ \\ 
         \hline
          
          \hline 
    \end{tabular}
    \end{adjustbox}
    \caption{Efficiency and information analysis of emergent codes and reference distribution. For each metric, we report the mean value and the standard variation when relevant (across seeds when experimenting with emergent languages and Monkey Typing and across the natural languages presented in Section \ref{section:method:ref2} for  Mean natural languages). `/' indicates that the metric cannot be computed. For $p_{\alpha}$, `*' indicates that the p-value is significant ($<0.001$). }
    \label{tab:metrics}
\end{table*}

In this section, we first reproduce and characterize the anti-efficient phenomenon that occurs with Standard Agents. Then, when experimenting with LazImpa, we show that this new communicative system leads to near-optimal and ZLA-compatible languages. Eventually, we demonstrate how both Impatience and Laziness are required to get an efficient communication protocol. 

All the quantitative results of the considered codes are gathered in Table \ref{tab:metrics}.

\subsection{Anti-efficient code with Standard Agents}
\label{section:results:std2}

We consider now Standard Agents and show how they develop inefficient code, of length close to \verb+max_len+. Moreover, their code is characterized by an inefficient allocation of information: with a low information density $\rho_{inf}$. Actually, only a very small proportion of the symbols localized at the end of the messages are informative.

\paragraph{Anti-ZLA communications.}

As shown in Figure~\ref{fig:ZLAN}, we reproduce \citet{chaabouni:etal:2019}'s result. In particular, our emergent languages have length distributions almost constant and close to the maximum length we set (=30): $L_{uni}$=$29.6$ and $L_{weight}$=$29.9$. The emergent codes are even less efficient than the random reference, Monkey Typing. On top of being inefficient, they also show an anti-ZLA pattern (see Appendix \ref{appendix:quantif} for quantitative support of this claim).%. The randomization test (see Appendix \ref{appendix:quantif} \mathieu{dans l'appendix définir le test réciproque de l'anti-ZLA}) shows that $L_{weight}$ is significantly higher than any other mean weighted message length obtained by permuting the frequency-length mapping ( $p_{\alpha}>1-10^{-5}$).

To bring some insights about this length anti-efficiency, we analyzed how the average length of the messages evolves during training. In Appendix \ref{appendix:learning_path}, we demonstrate that agents tend to explore long messages very quickly. In fact, at the beginning of the learning process, the messages are short and the accuracy is low. Then, when, and only when, the messages become long, communication starts to become successful. These results suggest that the exploration of long messages is key for the agents to succeed in the game, even though, in theory, shorter messages are sufficient. 

\begin{figure}[h] 
    \centering
    \includegraphics[scale=0.43]{figures/fig3_ZLA_HQ_lazimpa.png}
    \caption{Average message length across successful runs as a function of input frequency rank. %Emergent codes: blue curve refers to LazImpa, green curve to Standard Agents (light intervals show 1 standard deviation). Reference codes: grey curve refers to the Monkey Typing distribution, light green curve to English (curve smoothed by averaging 20 consecutive lengths) and purple curve to Optimal Coding.
    } 
    \label{fig:ZLAN}
\end{figure} 

\paragraph{Inefficient allocation of information.}

\begin{figure*}[h]
\begin{subfigure}[t]{.85\textwidth}
    \centering
    \hfill
    \begin{subfigure}[t]{.45\textwidth}
    \hspace{.5cm}
    \includegraphics[width=0.8\textwidth]{figures/spectrum_N_HQ2.jpg}
    \caption{Standard Agents \vspace{.2cm}}
    \label{fig:posNN}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.45\textwidth}
    \hspace{.5cm}
    \includegraphics[width=0.8\textwidth]{figures/spectrum_ILR_HQ.png}
    \caption{LazImpa \vspace{.2cm}}
    \label{fig:posIRLN}
    \end{subfigure}
    \hfill \\
    
    \hfill
    \begin{subfigure}[t]{.45\textwidth}
    %\hspace{.001mm}
    \hspace{.58cm}
    \includegraphics[width=0.8\textwidth]{figures/spectrum_NR_HQ.png}
    \caption{Lazy Speaker + Standard Listener}
    \label{fig:posNR}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.45\textwidth}
    %\hspace{.001mm}
    \hspace{.58cm}
    \includegraphics[width=0.8\textwidth]{figures/spectrum_IL_HQ.png}
    \caption{Standard Speaker + Impatient Listener}
    \label{fig:posILN}
    \end{subfigure}
    \hfill
\end{subfigure}
\hfill
\begin{subfigure}[c]{.05\textheight}
    \bigbreak
    \bigbreak
    \includegraphics[scale=0.2]{figures/gradient_HQ.png}
\end{subfigure}
\caption{Fraction of informative symbols at each position k averaged across all emergent messages of successful runs ($(\Lambda_{k,.})_{0\leq k \leq29}$). Each box represents the proportion of informative symbols at a given position $\Lambda_{k,.}$ mapped to a color according to a gray gradient (black=0 ; white=1). The red lines mark the mean message length $L_{uni}$ across successful run.}
    \label{fig:position_compaN}
\end{figure*}

%In Figure \ref{fig:position_compaN} (\rahma{only refer to 4a from the beginning. The explanation is in the title. Only one sentence to explain the figure would be enough}), we plot spectra that show how `informative' the different positions are by introducing a gray gradient that maps $\Lambda_{k,.}$ (information density of the $k^{th}$ symbol) to a color that goes from black ($\Lambda_{k,.}=0$) to white ($\Lambda_{k,.}=1$).

Looking  at the spectrum of Standard Agents in Figure \ref{fig:posNN}, we can make two striking observations. First,  only a very small part of the messages are actually informative (on average $\rho_{inf}=11\%$). Therefore, even if long messages seem necessary for the agents to succeed, most of the symbols are not used by Listener. In particular, if $L_{uni}=29.91$ on average, the average number of symbols used by Standard Listener ($L_{eff}$) is only equal to $3.33$ (which is even smaller than natural languages' mean message length $L_{uni}=5.46$). 
Surprisingly, we also observe that, if we restrict the messages to their informative symbols (i.e. removing positions $k$ with  $\Lambda_{k,.}=0$), the length statistics follow a ZLA-like distribution(see Figure \ref{fig:info_ZLA} in Appendix \ref{appendix:info_analysis}). Second, in all our experiments, the information is localized at the very end of the messages. That is, there is no actual information in the messages about Speaker's inputs before the last symbols. %\mathieu{je pense qu'il faut nuancer. Ici on dit que le Listener est passif. On peut tout aussi bien dire, `Listener attend que Speaker blablate jusqu'à la fin des messages où il commence à batir sa prédiction`}
\bigbreak
In sum, our analysis demonstrates that Standard Agents use actually efficient and  ZLA-like \emph{effective} communicative protocol. However, they make it maximally long adding non-informative symbols at the beginning of each message.

\subsection{Efficient code with LazImpa}
\label{section:results:LazImpa2}

Contrary to Standard Agents, the small variations introduced in the LazImpa system leads to the emergence of an efficient code. The latter follows ZLA and is characterized by a high information density $\rho_{inf}$. The resulting languages are moreover close to natural languages both in terms of length statistics and symbols distribution. However, agents do not manage to reach optimality. 

\paragraph{ZLA communication.}

LazImpa develops an efficient communication as presented in Figure \ref{fig:ZLAN}. Indeed, the average length of the messages is significantly lower than the Standard Agents system and Monkey Typing baseline (see also Table~\ref{tab:metrics}). Besides, we see that the length distribution follows ZLA: the shortest messages are associated to the most frequent inputs. The randomization test gives quantitative support of this observation ($p_{\alpha}<10
^{-5}$). 

\paragraph{Efficient allocation of information.}
We also look at information allocation when experimenting with LazImpa. In Table~\ref{tab:metrics}, we observe that Impatient Listener relies on $\rho_{inf}=60\%$ of the symbols. This corresponds to a big increase compared to $\rho_{inf}=19\%$ when using Standard Agents. However, we are still far from the $100\%$ observed in Optimal Coding. That is, even in the presence of a length cost (with Lazy Speaker), we still encounter non-informative symbols. Interestingly, as shown in Figure \ref{fig:posIRLN}, in contrast to Standard Agents, these informative symbols are localized in the first positions. By analyzing the intermediate predictions of Impatient Listener, we see that this model is actually able to guess the right input only reading approximately the $L_{eff}$ first positions (see Appendix \ref{appendix:min_length} for details).

\paragraph{Comparison with natural languages. }

\begin{figure*}[h]
    \begin{subfigure}[t]{.46\textwidth}
    \centering
    \includegraphics[scale=0.25]{figures/compa_NL_HQ.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.46\textwidth}
    \centering
    \includegraphics[scale=0.25]{figures/unigrams_HQ.png}
    \end{subfigure}
    \begin{subfigure}{1.\textwidth}
    \centering
    \includegraphics[scale=0.7]{figures/legende_nat_lang_LazImpa.png}
    \end{subfigure}
    \\
    \begin{subfigure}{.46\textwidth}
    \caption{Message length of natural languages and emergent languages (averaged across successful runs) as a function of input frequency rank. For readability, the curves have been smoothed using a sliding average of 20 consecutive lengths, see the real curves in Appendix \ref{appendix:stat_NL}. The light blue interval shows 1 standard deviation for the emergent language distribution.}
    \label{fig:compa_lenN}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.46\textwidth}
    \caption{Unigrams distribution of natural languages and emergent languages (averaged across successful messages) ranked by unigram frequency. The light blue interval shows 1 standard deviation for the emergent language unigrams distribution. \mathieu{mettre une footnote avec la ref du corpus des unigrams}}
    \label{fig:compa_uniN}
    \end{subfigure}
    \vspace{-.5cm}
    \caption{Comparison of the Emergent Language statistics and natural languages.}
    \label{fig:compa_NLN}
\end{figure*}

We demonstrated how LazImpa leads to the emergence of a ZLA-obeying code. In this part, we compare it to natural languages.
We see in Figure \ref{fig:compa_lenN} that the message lengths in the emergent communication are, in average, analogous to the words lengths in natural languages: $L_{uni}$ are in average the same, while $L_{weight}$ are also very close ($L_{weight}=3.78$ for emergent codes while $L_{weight}=3.55$ for natural languages). We further compare their unigram distributions. \citet{chaabouni:etal:2019} showed that Standard Agents develop repetitive messages with a skewed unigram distribution. Our results, in Figure \ref{fig:compa_uniN}, show that, on top of a ZLA-like code, LazImpa enables the emergence of natural-language-like unigram distribution, without any particular repetitive pattern. Intriguingly, this similarity with natural languages is an unexpected property as a uniform distribution of unigrams would lead to a more efficient protocol.


\paragraph{Comparison with Optimal Coding. }

If LazImpa leads to significantly more efficient languages compared to Standard Agents, these emergent languages are still not as efficient as Optimal Coding (see Figure \ref{fig:ZLAN}). First, we can note that the informative length $L_{eff}$ is slightly sub-optimal ($L_{eff}=2.67$ for LazImpa, $L_{eff}=1.96$ for Optimal Coding). This difference can be explained by the non-uniform use of unigrams. We show in Appendix \ref{appendix:min_length} that LazImpa languages approximate Optimal Coding (w.r.t. $L_{eff}$) when the latter uses the same skewed unigram distribution. A second source of sub-optimality %, the persisting difference between LazImpa and Optimal codes 
comes from the addition of uninformative symbols at the end of the messages (as detailed above). This phenomenon is still unexplained and we leave the analysis of reaching optimal communication to future works.

\subsection{Ablation study}
\label{section:results:compamodels2}

\begin{figure*}[h]
    \begin{subfigure}[t]{.46\textwidth}
    \centering
    \includegraphics[scale=0.23]{figures/learning_path_HQ.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.46\textwidth}
    \centering
    \includegraphics[scale=0.25]{figures/ZLA_compa_model_HQ_n.png}
    \end{subfigure}
    \begin{subfigure}{1.\textwidth}
    \centering
    \includegraphics[width=0.92\textwidth]{figures/legende_modele_compa_lazimpa.png}
    \end{subfigure}
    \\
    \begin{subfigure}{.46\textwidth}
    \caption{Joint evolution of the accuracy and mean length for the different models. Each point shows the couple (mean length,accuracy) of one training episode. Arrows represent the average joint evolution of the two variables.}
    \label{fig:compa_learning_pathN}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.46\textwidth}
    \caption{Average message length as a function of input frequency rank for the different systems. Light color intervals show 1 standard deviation.}
    \label{fig:compa_lengthN}
    \end{subfigure}
    \vspace{-.5cm}
    \caption{Comparison of different communication systems.%In both figures, the green curve refers to the system (Standard Speaker + Standard Listener), the red curve to the system (Reg. Speaker + Standard Listener), the orange curve to the system (Standard Speaker + Imp. Listener), the blue curve to the system (Reg. Speaker + Standard Impatient)
    } 
\end{figure*}

We have just seen that our new communication system LazImpa allows agents to develop an efficient and ZLA-obeying language whose statistical properties are close to those of natural languages. In this section, we analyze the effects of the modeling choices we have made.

We first look at the effect of Laziness. To do so, we compare LazImpa to the system (Standard Speaker + Impatient Listener) (i.e. removing the length regularization). Figure \ref{fig:compa_learning_pathN} shows the joint evolution of the mean length of messages ($L_{uni}$) and game accuracy. We observe that our non-regularized system, similarly to LazImpa, initially explores long messages  while being more successful (exploration step). Surprisingly, even in the absence of Laziness, the exploration step does not continue to maximally long messages, as it is the case for Standard Agents, but breaks at length $\approx 20$. However, \emph{contrary to LazImpa}, (Standard Speaker + Impatient Listener) does not present an ablation step (a reduction of mean length for a fixed good accuracy). Thus, as expected, the introduction of Laziness in LazImpa is responsible for the ablation step, and hence for shorter and more efficient communication protocol. However, we note in Figure \ref{fig:compa_lengthN}, that Impatience alone is sufficient for the emergence of ZLA. Moreover, when looking at the information spectrum, comparing (Standard Speaker + Impatient Listener) (Figure \ref{fig:posILN}) to LazImpa (Figure \ref{fig:posIRLN}), we observe how alike both systems allocate information and differ only by their mean length.

Second, we investigate the role of Impatience. We see in Figure \ref{fig:compa_learning_pathN} that the system (Lazy Speaker + Standard Listener) admits a visually different dynamic compared to LazImpa. In particular, the exploration step leads to significantly longer messages, close to \verb+max_len+. Interestingly, if we demonstrated above the necessity of Laziness for the ablation step, alone, it does not induce it: no ablation step in the (Lazy Speaker + Standard Listener) system is observed. This is due to the necessity of long messages when experimenting with Standard Listener. Specifically, as informative symbols are present only at the last positions (see Figure \ref{fig:posNR}), introducing a length regularization provokes a drop in accuracy, which in turn cancels the regularization. In other words, the length regularization scheduling stops at the exploration step, which makes the system almost equivalent to Standard Agents (this could be also seen experimentally  in Figures \ref{fig:compa_learning_pathN} and \ref{fig:compa_lengthN}).

Taken together, our analysis emphasizes the importance of both Impatience \emph{and} Laziness for the emergence of efficient communication.

